DAP: Diffusion-based Affordance Prediction for Multi-modality Storage

Solving storage problem: where objects must be accurately placed into containers with precise orientations and positions, presents a distinct challenge that extends beyond traditional rearrangement tasks. These challenges are primarily due to the need for fine-grained 6D manipulation and the inherent multi-modality of solution spaces, where multiple viable goal configurations exist for the same storage container. We present a novel Diffusion-based Affordance Prediction (DAP) pipeline for the multi-modal object storage problem. DAP leverages a two-step approach, initially identifying a placeable region on the container and then precisely computing the relative pose between the object and that region. Existing methods either struggle with multi-modality issues or computation-intensive training. Our experiments demonstrate DAP's superior performance and training efficiency over the current state-of-the-art RPDiff, achieving remarkable results on the RPDiff benchmark. Additionally, our experiments showcase DAP's data efficiency in real-world applications, an advancement over existing simulation-driven approaches. Our contribution fills a gap in robotic manipulation research by offering a solution that is both computationally efficient and capable of handling real-world variability. Code and supplementary material can be found at: https://github.com/changhaonan/DPS.git.

==> experiment_new.tex <==
\section{EXPERIMENTS}

We conduct a comprehensive series of experiments, aiming to address two key questions: (1) How does the performance of DAP compare with other methods? (2) How crucial is the diffusion-based affordance prediction for addressing the multi-modality issue? 

\subsection{Simulation Experiment} 
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/rpdiff_dataset.png}
    \caption{\small{Samples from RPdiff benchmark. We show two sample scenes from RPdiff benchmark: one is placing a book into the bookshelf and the other is to stack a can inside an cabinet. }}
    \label{fig:corr}
\end{figure}
We evaluate our method using the benchmark from RPDiff~\cite{shelving}, which provides a challenging simulation environment for addressing the multi-modal rearrangement problem. This environment includes tasks such as book shelving, can stacking, and cup hanging, all of which highlight the benchmark's complexity due to the variability in container and object geometries within each task. This variability demands a model's ability to generalize across different geometric configurations. We exclude the cup hanging task from evaluation as it does not match our problem requirement that the object is to be placed in a bigger container.
The benchmark's inputs are a container point cloud $\mathbf{P}_C$ and an object point cloud $\mathbf{P}_O$. Success is determined by the object's stable placement inside the container. The reported success rate is averaged over 100 independent random trials.

Regarding the baselines, we adopt the same benchmarks used in RPDiff~\cite{shelving}. We compare our approach against five baseline methods, each offering a unique perspective on tackling multi-modal rearrangement problems:

\noindent \textbf{Coarse-to-Fine Q-attention (C2F-QA):} Adapted from a classification approach, this method predicts a score distribution over a voxelized scene representation to identify candidate translations of the object centroid. It operates in a coarse-to-fine manner, refining predictions at higher resolutions and culminating in a rotation prediction for the object. The best-scoring transformation is then executed.

\noindent \textbf{Relational Neural Descriptor Fields (R-NDF):} Utilizing a neural field shape representation, R-NDF matches local coordinate frames to category-level 3D models, facilitating relational rearrangement tasks. The ``R-NDF-base" version does not include the refinement energy-based model found in the original implementation.

\noindent \textbf{Neural Shape Mating (NSM) + CVAE:} NSM processes paired point clouds via a Transformer to align them. The ``NSM-base" differs in its training on large perturbations without local cropping and makes a single prediction. To address multi-modality, NSM is enhanced with a Conditional Variational Autoencoder (CVAE), allowing for multiple transform predictions, with the top-scoring transform selected for execution. ``NSM-base" and ``NSM-base + CVAE" are considered as two different baselines.

\noindent \textbf{Relational Pose Diffusion (RPDiff):} RPDiff operates directly on 3D point clouds and is capable of generalizing across novel geometries, poses, and layouts. It addresses the challenge of multiple similar rearrangement solutions through an iterative pose de-noising training strategy, allowing for precise, multi-modal outputs. It was the state of the art method on RPDiff's benchmark until the present work.
% By focusing on local geometric features and disregarding irrelevant global structures, RPDiff ensures enhanced generalization and accuracy across various rearrangement tasks in both simulation and real-world scenarios.

% \noindent\includegraphics[width=\linewidth]{example-image} 

\begin{table}[]
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method}     & \textbf{Book/Shelf} & \textbf{Can/Cabinet} \\ \midrule
C2F Q-attn          & 57$\%$                & 51$\%$                 \\
R-NDF-base          & 00$\%$                & 14$\%$                 \\
NSM-base            & 02$\%$                & 08$\%$                 \\
NSM-base + CVAE     & 17$\%$                & 19$\%$                 \\
RPDiff              & 94$\%$                & 85$\%$                 \\
\textbf{DAP (ours)} & \textbf{98}$\%$                    &  \textbf{94}$\%$                    \\ \bottomrule
\end{tabular}
\caption{Performance on RPDiff benchmark (Success rate).} \label{tab:performance}
\end{table}

The comparative performance of DAP and the baselines is presented in TABLE~\ref{tab:performance}. The table illustrates that RPDiff significantly outperforms the other four baselines. However, DAP exceeds RPDiff's performance by a considerable margin, highlighting DAP's superior capability. Furthermore, the efficiency of DAP is demonstrated through its training requirements: RPDiff necessitates three days of training on a V100 GPU for its action module and an additional five days for the evaluation module on each task. In contrast, DAP requires only one hour for training the affordance prediction module and another hour for pose estimation, all on a single 3090 GPU, showcasing DAP's remarkable efficiency.

\begin{table}[]
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method}     & \textbf{Book/Shelf} & \textbf{Can/Cabinet} \\ \midrule
CAP          &  24$\%$      &     36$\%$   \\ 
\textbf{DAP (ours)} & \textbf{98}$\%$                    &  \textbf{94}$\%$           \\ \bottomrule
\end{tabular}
\caption{Ablation study on RPDiff benchmark.} \label{tab:ablation}
\end{table}

\subsection{Ablation Study}
To analyze the impact of diffusion-based affordance prediction, we conducted an ablation study upon RPDiff benchmark. We compare DAP with a variant framework without using DDPM loss:

\noindent \textbf{Classification Affordance Prediction (CAP):} Instead of treating affordance prediction as a generative task, we approach it as a classification problem using cross-entropy loss. The architecture remains the same as DAP. During inference we do not perform iterative de-noising, but provide the classification in one step.

% \noindent \textbf{Direct Pose Estimation (DPE):} Instead of utilizing correspondence prediction combined with Arun's algorithm for pose determination, we examine a variant of DAP that directly outputs pose estimation. We adapt our architecture, as shown in Fig.~\ref{fig:corr}, by eliminating the correspondence matrix prediction and incorporating a pose decoder. This decoder predicts the translation vector and rotation axis, which previous work~\cite{sundermeyer2023bop} has shown to be effective and stable.

The results of our ablation study are depicted in TABLE~\ref{tab:ablation}. Classification Affordance Prediction (CAP) significantly under-performs compared to the complete DAP. This finding confirms our hypothesis that diffusion-based affordance prediction effectively addresses multi-modality issues.

\subsection{Limitation \& Future Direction}
Currently, DAP is primarily limited to storage problems, wherein a target object is placed inside a larger container. In this setup, after applying the diffusion-based affordance segmentation to the container's point cloud, there is only one optimal goal pose for the local region. For tasks where multiple optimal solutions exist within the local region, such as hanging a cup, which can be hung by its handle or by its rim, DAP performs less effectively. Investigating how to combine diffusion model with correspondence prediction can be a future research direction.
